ALMA Polarization Study of the Magnetic Fields in Two Massive Clumps in the 20 km s$^{-1}$ Cloud of the Central Molecular Zone

We present the Atacama Large Millimeter/submillimeter Array (ALMA) observations of linearly polarized 870 $\mu$m continuum emission at a resolution of $\sim$0.2$^{\prime\prime}$ (2000 au) toward the two massive clumps, Clump 1 and Clump 4, in the 20 km s$^{-1}$ cloud. The derived magnetic field strengths for both clumps range from $\sim$0.3 to 3.1 mG using the Angular Dispersion Function (ADF) method. The magnetic field orientations across multiple scales suggests that the magnetic field dominates at the cloud scale, whereas gravity likely governs the structures at the core (0.01$-$0.1 pc) and condensation ($\le$ 0.01 pc) scales. Furthermore, the study on the angular difference between the orientations of the local gravity gradient and the magnetic field suggests that the gravity predominantly governs the dynamics in the diffuse regions, while both gravity and star formation feedback become increasingly significant within the dense regions. The ratio of the magnetic field tension force $F_\mathrm{B}$ to the gravitational force $F_\mathrm{G}$ suggests that the magnetic field may provide some support against gravity, but it is insufficient to prevent gas from infalling toward the dense cores.

==> authors.tex <==

\author[0009-0009-2263-5502]{Yuhua Liu (柳玉华)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\email{liuyuhua@shao.ac.cn}

% Main contributors to the paper
\author[0000-0003-2619-9305]{Xing Lu (吕行)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\affiliation{State Key Laboratory of Radio Astronomy and Technology, A20 Datun Road, Chaoyang District, Beijing, 100101, P.\ R.\ China}
\email{xinglu@shao.ac.cn}


\author[0000-0002-4774-2998]{Junhao Liu (刘峻豪)}
\affiliation{National Astronomical Observatory of Japan, 2-21-1 Osawa, Mitaka, Tokyo, 181-8588, Japan}
\email{liujunhao42@outlook.com}


\author[0000-0003-1337-9059]{Xing Pan (潘兴)}
\affiliation{School of Astronomy and Space Science, Nanjing University, 163 Xianlin Avenue, Nanjing 210023, P.R.China}
\affiliation{Key Laboratory of Modern Astronomy and Astrophysics (Nanjing University), Ministry of Education, Nanjing 210023, P.R.China}
\affiliation{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA, 02138, USA}
\email{xingpan1017@gmail.com}

% Proposal PI
\author[0000-0003-2384-6589]{Qizhou Zhang}
\affiliation{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA, 02138, USA}
\email{qzhang@cfa.harvard.edu}


% Other people who have make substantial contributions
\author[0000-0003-2300-2626]{Hauyu Baobab Liu}
\affiliation{Department of Physics, National Sun Yat-Sen University, No. 70, Lien-Hai Road, Kaohsiung City 80424}
\affiliation{Center of Astronomy and Gravitation, National Taiwan Normal University, Taipei 116}
\email{baobabyoo@gmail.com}

\author[0009-0003-5699-2723]{Meng-Zhe Yang}
\affiliation{Institute of Astronomy and Department of Physics, National Tsing Hua University, Hsinchu 30013, Taiwan}
\email{jeremys93102@gapp.nthu.edu.tw}


\author[0000-0001-5522-486X]{Shih-Ping Lai}
\affiliation{Institute of Astronomy and Department of Physics, National Tsing Hua University, Hsinchu 30013, Taiwan}
\email{slai@gapp.nthu.edu.tw}

\author[0000-0001-8516-2532]{Tao-Chung Ching}
\affiliation{National Radio Astronomy Observatory, P.O. Box O, Socorro, NM 87801, USA}
\email{chingtaochung@gmail.com}

\author[0000-0001-9822-7817]{Wenyu Jiao (焦文裕)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\email{wenyujiao@shao.ac.cn}

\author[0000-0001-7817-1975]{Yankun Zhang (张燕坤)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\email{zhangyankun@shao.ac.cn}

\author[0000-0001-8077-7095]{Pak Shing Li}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\email{pakshingli@shao.ac.cn}

\author[0000-0003-3540-8746]{Zhiqiang Shen (沈志强)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\affiliation{State Key Laboratory of Radio Astronomy and Technology, A20 Datun Road, Chaoyang District, Beijing, 100101, P.\ R.\ China}
\email{zshen@shao.ac.cn}

\author[0000-0002-5286-2564]{Tie Liu (刘铁)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\affiliation{State Key Laboratory of Radio Astronomy and Technology, A20 Datun Road, Chaoyang District, Beijing, 100101, P.\ R.\ China}
\email{liutie@shao.ac.cn}



\author[0000-0001-7817-1975]{Adam Ginsburg}
\affiliation{University of Florida Department of Astronomy, Bryant Space Science Center, Gainesville, FL, 32611, USA}
\email{adamginsburg@ufl.edu}

\author[0000-0002-2826-1902]{Qi-lao Gu (顾琦烙)}
\affiliation{Shanghai Astronomical Observatory, Chinese Academy of Sciences, 80 Nandan Road, Shanghai 200030, P.\ R.\ China}
\email{qlgu@shao.ac.cn}

\author[0000-0003-0596-6608]{Mengke Zhao}
\affiliation{South-Western Institute for Astronomy Research, Yunnan University, Chenggong District, Kunming 650500, China}
\affiliation{School of Astronomy and Space Science, Nanjing University, 163 Xianlin Avenue, Nanjing 210023, People’s Republic of China}
\email{mkzhao628@gmail.com}


%\author[0000-0003-2133-4862]{Thushara Pillai}
%\affiliation{Haystack Observatory, Massachusetts Institute of Technology, 99 Millstone Road, Westford, MA 01886, USA}

%\author[0000-0002-5094-6393]{Jens Kauffmann}
%\affiliation{Haystack Observatory MIT, 99 Milstone Rd, Westford, MA 01886, USA}

%\author[0000-0001-7330-8856]{Daniel Walker}
%\affiliation{UK ALMA Regional Centre Node, Jodrell Bank Centre for Astrophysics, The University of Manchester, Manchester M13 9PL, UK}
%\affiliation{Department of Physics, University of Connecticut, 196A Auditorium Road, Storrs, CT 06269, USA}


%\author[0000-0001-6353-0170]{Steven N. Longmore}
%\affiliation{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}
%\affiliation{Cosmic Origins Of Life (COOL) Research DAO, Germany}


%\author[0000-0002-6073-9320]{Cara Battersby}
%\affiliation{Department of Physics, University of Connecticut, 196A Auditorium Road, Storrs, CT 06269, USA}
%\affiliation{Center for Astrophysics $\vert$ Harvard \& Smithsonian, 60 Garden Street, Cambridge, MA, 02138, USA}

%\author[0000-0001-8782-1992]{Elisabeth A. C. Mills}
%\affiliation{Department of Physics and Astronomy, University of Kansas, 1251 Wescoe Hall Drive, Lawrence, KS 66045, USA}

%\author[0000-0002-8804-0212]{J. M. Diederik Kruijssen}
%\affiliation{Cosmic Origins Of Life (COOL) Research DAO, Germany}

% Proposal co-Is

% SHAO people
